Petrification: Software Model Checking for Programs with Dynamic Thread Management (Extended Version)

We address the verification problem for concurrent program that dynamically create (fork) new threads or destroy (join) existing threads. We present a reduction to the verification problem for concurrent programs with a fixed number of threads. More precisely, we present petrification, a transformation from programs with dynamic thread management to an existing, Petri net-based formalism for programs with a fixed number of threads. Our approach is implemented in a software model checking tool for C programs that use the pthreads API.

==> sections/boogie-extension.tex <==
% !TEX root = ../main.tex

\section{Boogie and Semantics}
%
(this section should be rather short)

\begin{itemize}
  \item our tool extends Boogie; for lack of space we only present here a fragment relevant for concurrency; possibly link web interface for full
  \item give Boogie syntax, including concurrency extensions
    (we do not introduce call/return but mention our implementation supports it; procedures are still used as thread templates; fork maybe only with a single thread id (not a list); if necessary cut more like e.g. \texttt{goto})
  \item give semantics to sequential fragment
  \item proposition: this is equivalent to original Boogie semantics
  \item extend semantics to concurrent Boogie programs
\end{itemize}
